Keeping Designers in the Loop: Communicating Inherent Algorithmic Trade-offs Across Multiple Objectives

Artificial intelligence algorithms have been used to enhance a wide variety of products and services, including assisting human decision making in high-stakes contexts. However, these algorithms are complex and have trade-offs, notably between prediction accuracy and fairness to population subgroups. This makes it hard for designers to understand algorithms and design products or services in a way that respects users' goals, values, and needs. We proposed a method to help designers and users explore algorithms, visualize their trade-offs, and select algorithms with trade-offs consistent with their goals and needs. We evaluated our method on the problem of predicting criminal defendants' likelihood to re-offend through (i) a large-scale Amazon Mechanical Turk experiment, and (ii) in-depth interviews with domain experts. Our evaluations show that our method can help designers and users of these systems better understand and navigate algorithmic trade-offs. This paper contributes a new way of providing designers the ability to understand and control the outcomes of algorithmic systems they are creating.

==> DIS 20 - Algorithm Trade-off Explanation/math.tex <==
To show trade-offs between disparity and prediction errors, we reduced it to a sequence of cost-sensitive classification (CSC) problems, and the solutions to it yield a randomized classifier $Q$ with the lowest (empirical) error subject to the desired constraints, see equation (2).
\begin{equation}
    \begin{aligned}
        L(Q, \lambda_0, \lambda_1) = &  \hspace{2mm} err(Q) \\
        & + \lambda_0 (FP(a_1) - FP(a_0)) \\
        % \sum_{i=1}^{n} (\mathds{1}[ \^{Y}_i=1, Y_i=0, a_i=1] - \mathds{1}[ \^{Y}_i=1, Y_i=0, a_i=0]) \\
        & + \lambda_1 (FN(a_1) - FN(a_0)). 
        %\sum_{i=1}^{n} (\mathds{1}[ \^{Y}_i=0, Y_i=1, a_i=1] - \mathds{1}[ \^{Y}_i=0, Y_i=1, a_i=0])
    \end{aligned}
\end{equation}

The input to such a CSC algorithm is a data set of training examples $\{(X_i, C_i^0, C_i^1)\}_{i=1}^n$, where $C_i^0$ and $C_i^1$ denotes the costs of predicting label 1 and 0 (the defendant to reoffend or not), respectively, for $X_i$:
\begin{equation}
    \operatorname*{argmin}_{h\in Q} \sum_{i=1}^{n} h(x_i)C^1_i + (1-h(x_i))C^0_i.
\end{equation}

Thus, we can incorporate fairness constraints by specifying different costs for different training examples. In particular, equation (2) is equivalent to a weighted classification problem, where the input consists of labeled examples $\{(X_i, Y_i, W_i)\}_{i=1}^n$ with $Y_i \in \{0, 1\}$ and $W_i \geq 0$, and the goal is to minimize the weighted classification errors:
\begin{equation}
    \operatorname*{argmin}_{h\in Q}\sum_{i=1}^{n} W_i\textbf{1}\{h(X_i)\neq Y_i\}.
\end{equation}

This is equivalent to equation (2) if we set $W_i = |C_i^0 - C_i^1|$ and $Y_i=\textbf{1}\{C_i^0 \geq C_i^1\}$, where the costs, $C_i^0$ and $C_i^1$, can be written as the following:
\begin{equation}
    \begin{aligned}
        C^0_i = \mathds{1} [Y_i=1] + \lambda_1 
        (\mathds{1}[ Y_i=1, a_i=1] - \mathds{1}[ Y_i=1, a_i=0]), \\
        C^1_i = \mathds{1} [Y_i=0] + \lambda_0 
        (\mathds{1}[ Y_i=0, a_i=1] - \mathds{1}[ Y_i=0, a_i=0]).
    \end{aligned}
\end{equation}



Since we constrained the problem to only consider binary protected attributes (African and White defendants, male and female defendants), it is suffices to conduct grid search on values of $\lambda_1$ and $\lambda_2$ to calculate the best response for each pair of values, and select values with the desired trade-offs between prediction errors and disparity by generating the Pareto frontier (see Figure \ref{fig:tradeoffs_disp_error}). 

% range of lambda1 and lambda2??

To solve the binary classification in the cost-sensitive classification problem, we used logistic regression for each $h \in Q$, because logistic regression can provide the probability of each label on each example which allows  for thresholding to display trade-offs between the two types of prediction errors.

==> math.tex <==
To show trade-offs between disparity and prediction errors, we reduced it to a sequence of cost-sensitive classification (CSC) problems, and the solutions to it yield a randomized classifier $Q$ with the lowest (empirical) error subject to the desired constraints, see equation (2).
\begin{equation}
    \begin{aligned}
        L(Q, \lambda_0, \lambda_1) = &  \hspace{2mm} err(Q) \\
        & + \lambda_0 (FP(a_1) - FP(a_0)) \\
        % \sum_{i=1}^{n} (\mathds{1}[ \^{Y}_i=1, Y_i=0, a_i=1] - \mathds{1}[ \^{Y}_i=1, Y_i=0, a_i=0]) \\
        & + \lambda_1 (FN(a_1) - FN(a_0)). 
        %\sum_{i=1}^{n} (\mathds{1}[ \^{Y}_i=0, Y_i=1, a_i=1] - \mathds{1}[ \^{Y}_i=0, Y_i=1, a_i=0])
    \end{aligned}
\end{equation}

The input to such a CSC algorithm is a data set of training examples $\{(X_i, C_i^0, C_i^1)\}_{i=1}^n$, where $C_i^0$ and $C_i^1$ denotes the costs of predicting label 1 and 0 (the defendant to reoffend or not), respectively, for $X_i$:
\begin{equation}
    \operatorname*{argmin}_{h\in Q} \sum_{i=1}^{n} h(x_i)C^1_i + (1-h(x_i))C^0_i.
\end{equation}

Thus, we can incorporate fairness constraints by specifying different costs for different training examples. In particular, equation (2) is equivalent to a weighted classification problem, where the input consists of labeled examples $\{(X_i, Y_i, W_i)\}_{i=1}^n$ with $Y_i \in \{0, 1\}$ and $W_i \geq 0$, and the goal is to minimize the weighted classification errors:
\begin{equation}
    \operatorname*{argmin}_{h\in Q}\sum_{i=1}^{n} W_i\textbf{1}\{h(X_i)\neq Y_i\}.
\end{equation}

This is equivalent to equation (2) if we set $W_i = |C_i^0 - C_i^1|$ and $Y_i=\textbf{1}\{C_i^0 \geq C_i^1\}$, where the costs, $C_i^0$ and $C_i^1$, can be written as the following:
\begin{equation}
    \begin{aligned}
        C^0_i = \mathds{1} [Y_i=1] + \lambda_1 
        (\mathds{1}[ Y_i=1, a_i=1] - \mathds{1}[ Y_i=1, a_i=0]), \\
        C^1_i = \mathds{1} [Y_i=0] + \lambda_0 
        (\mathds{1}[ Y_i=0, a_i=1] - \mathds{1}[ Y_i=0, a_i=0]).
    \end{aligned}
\end{equation}



Since we constrained the problem to only consider binary protected attributes (African and White defendants, male and female defendants), it is suffices to conduct grid search on values of $\lambda_1$ and $\lambda_2$ to calculate the best response for each pair of values, and select values with the desired trade-offs between prediction errors and disparity by generating the Pareto frontier (see Figure \ref{fig:tradeoffs_disp_error}). 

% range of lambda1 and lambda2??

To solve the binary classification in the cost-sensitive classification problem, we used logistic regression for each $h \in Q$, because logistic regression can provide the probability of each label on each example which allows  for thresholding to display trade-offs between the two types of prediction errors.
